Ferret: Refer and Ground Anything Anywhere at Any Granularity

We introduce Ferret, a new Multimodal Large Language Model (MLLM) capable of understanding spatial referring of any shape or granularity within an image and accurately grounding open-vocabulary descriptions. To unify referring and grounding in the LLM paradigm, Ferret employs a novel and powerful hybrid region representation that integrates discrete coordinates and continuous features jointly to represent a region in the image. To extract the continuous features of versatile regions, we propose a spatial-aware visual sampler, adept at handling varying sparsity across different shapes. Consequently, Ferret can accept diverse region inputs, such as points, bounding boxes, and free-form shapes. To bolster the desired capability of Ferret, we curate GRIT, a comprehensive refer-and-ground instruction tuning dataset including 1.1M samples that contain rich hierarchical spatial knowledge, with 95K hard negative data to promote model robustness. The resulting model not only achieves superior performance in classical referring and grounding tasks, but also greatly outperforms existing MLLMs in region-based and localization-demanded multimodal chatting. Our evaluations also reveal a significantly improved capability of describing image details and a remarkable alleviation in object hallucination. Code and data will be available at https://github.com/apple/ml-ferret

==> related_work.tex <==
\section{Related Work}
% \label{app:related_work}

\textbf{Multimodal large language models (MLLMs).}
Large Language Models (LLMs), including GPTs~\citep{brown2020language,gpt4}, PaLM~\citep{chowdhery2022palm}, BLOOM~\citep{scao2022bloom}, and LLaMA~\citep{touvron2023llama,touvron2023llama2}, have revolutionized research in NLP, spurring significant advances in multimodal language models as well. Early models primarily focused on large-scale image-text pre-training. Notable examples include SimVLM~\citep{wang2021simvlm}, GIT~\citep{wang2022git}, PaLI~\citep{chen2022pali}, PaLI-X~\citep{chen2023pali}, BLIP-2~\citep{li2023blip}, Flamingo~\citep{alayrac2022flamingo}, PaLM-E~\citep{driess2023palm}, CM3~\citep{aghajanyan2022cm3}, and CM3Leon~\citep{yu2023scaling}. Flamingo, in particular, pioneered the integration of a pre-trained CLIP image encoder with LLMs through gated cross-attention blocks, showcasing emergent multimodal in-context few-shot learning capabilities. Its open-sourced variants, such as OpenFlamingo~\citep{anas_awadalla_2023_7733589} and IDEFICS~\citep{laurenccon2023obelisc}, have garnered significant attention. Typically, these models undergo pre-training using millions or even billions of image-text pairs and interleaved image-text datasets~\citep{zhu2023multimodal}.

On the other hand, recent research has increasingly focused on using pre-trained LLMs for visual instruction tuning. Prominent examples include LLaVA~\citep{liu2023visual}, MiniGPT-4~\citep{zhu2023minigpt}, mPLUG-Owl~\citep{ye2023mplug}, Otter~\citep{li2023otter}, InstructBLIP~\citep{dai2023instructblip}, to name a few. In additional to text generation, recent models like FROMAGe~\citep{koh2023grounding}, GILL~\citep{koh2023generating}, Emu~\citep{sun2023generative}, have also enabled MLLMs for image retrieval and image generation. Please refer to Chapter 5 of \cite{li2023multimodal} for a detailed review. 

\textbf{MLLMs for referring and grounding.}
In the realm of existing literature, works such as Kosmos-2~\citep{peng2023kosmos} and Shikra~\citep{chen2023shikra},  closely resemble ours as they also enable MLLMs for fine-grained image comprehension and open-world referring and grounding. Additional works in this direction include  GPT4ROI~\citep{zhang2023gpt4roi}, BuboGPT~\citep{zhao2023bubogpt}, VisionLLM~\citep{wang2023visionllm}, and ContextDET~\citep{zang2023contextual}. Nevertheless, pivotal distinctions set our model apart.
First, prior endeavors supported only bounding boxes as both input and output. Conversely, due to Ferret's innovative hybrid region representation, we accommodate a broader range of free-form shapes for referring, encompassing points, boxes, sketches, scribbles, polygons, and more.
Second, we meticulously curate an extensive refer-and-ground instruction tuning dataset.
Third, we introduce Ferret-Bench to facilitate forthcoming research and enhance evaluation benchmarks in this direction.
Lastly, our model exhibits superior performance compared to previous works, notably mitigating object hallucination to a significant extent. 

\textbf{Unifying grounding and VL understanding.} Our work is also related to previous work that aims to unify text and bounding box output for vision-language (VL) models, such as UniTAB~\citep{yang2022unitab}, OFA~\citep{wang2022ofa}, and Unified-IO~\citep{lu2022unified}, which also represent bounding boxes using a set of additional discrete tokens as proposed in Pix2Seq~\citep{chen2021pix2seq,chen2022unified}. Ferret is unique in that ($i$) our model is built upon LLMs, marrying the power of LLMs and grounding, thus unlocking new capabilities such as grounded instruction tuning, and ($ii$) we handle bounding box coordinates as regular text tokens, avoiding the need for extra specialized tokens dedicated to representing boxes.

